Quantum algorithms for cooling: a simple case study

Preparation of low-energy quantum many-body states has a wide range of applications in quantum information processing and condensed matter physics. Quantum cooling algorithms offer a promising alternative to other methods based, for instance, on variational and adiabatic principles, or on dissipative state preparation. In this work, we investigate a set of cooling algorithms in a simple, solvable fermionic model which allows us to identify the mechanisms which underlie the cooling process and, also, those which prevent it. We derive analytical expressions for the cooling dynamics, steady states, and cooling rates in the weak coupling limit. We find that multi-frequency and randomized cycle strategies can significantly enhance the performance of the quantum algorithm and circumvent some of the obstacles. We also analyze the effects of noise and evaluate the conditions under which cooling remains feasible. Furthermore, we present optimized cooling protocols that can significantly enhance cooling performance in the presence of noise. Additionally, we compare cooling and dissipative state preparation and show that, in the model analyzed here, cooling generally achieves lower energies and is more resilient to noise.

==> newCoolingAppA.tex <==

\section{Derivation of the Mode-Dependent Hamiltonian}
\label{app:Hk_derivation}

In this appendix, we present the details about the block-diagonalization of the Hamiltonian considered in this work. We will first diagonalize the system Hamiltonian and then block-diagonalize the total Hamiltonian. Throughout this and other appendices, we will use dimensionless units for all energy scales and coupling constants.

% ------------------------------------------------------------
\subsection{System Hamiltonian}

The system will be composed of an even number, $N$, of fermionic modes. The system Hamiltonian is given by
\begin{align}
    H_S &= \frac{1}{2} \sin\theta \sum_{n=1}^N (a_n^\dagger a_n - a_n a_n^\dagger)\nonumber\\
        &\quad + \frac{1}{2} \cos\theta \sum_{n=1}^N [a_n^\dagger (a_{n+1} + i a_{n+1}^\dagger) + \text{h.c.}],
    \label{eq:app:system-hamiltonian}
\end{align}
where $a_n$ ($a_n^\dagger$) denotes the fermionic annihilation (creation) operator at site $n$, with the periodic boundary condition $a_{N+1} = a_{1}$.

As mentioned in \cref{subsec:sys_model} of the main text, the system Hamiltonian is traceless and possesses various symmetries, which allow us to restrict, without loss of generality, $\theta$ to the interval $[0,\pi/2]$. This will be further proved in \cref{app:theta_mapping}.

We now derive the momentum-space formulation of \cref{eq:app:system-hamiltonian}. We begin by introducing the Fourier transform for an even number $N$ of fermionic modes:
\begin{align}
    \tilde{a}_k         &= \frac{1}{\sqrt{N}} \sum_{n=1}^N e^{i \frac{2\pi k n}{N}} a_n,\\
    \tilde{a}_k^\dagger &= \frac{1}{\sqrt{N}} \sum_{n=1}^N e^{-i \frac{2\pi k n}{N}} a_n^\dagger.
\end{align}
The operators $\tilde{a}_k$ and $\tilde{a}_k^\dagger$ are defined to be the annihilation and creation operators in momentum space. These definitions can be inverted using the orthogonality relation $\sum_{n=1}^N e^{i \frac{2\pi (k-q) n}{N}} = N \delta_{k,q}$ to obtain
\begin{equation}
    \label{eq:fourier_def_ann}
    a_n = \frac{1}{\sqrt{N}} \sum_{k=-N/2+1}^{N/2} e^{-i \frac{2\pi k n}{N}}  \tilde{a}_k,
\end{equation}
and similarly for $a_n^\dagger$. Here, $k$ runs over integer values from $-N/2+1$ to $N/2$.

Expressing $H_S$ in terms of the new operators leads to:
\begin{equation}
    H_S=\sum_{k=1}^{N/2-1} \tilde{\alpha}_k^\dagger \tilde{H}_k \tilde{\alpha}_k+ H_{k=0}+H_{k=N/2}.
\end{equation}
Here, we defined for any $k$ such that $1 \le k \le N/2-1$ the vector
\begin{align}
    \tilde{\alpha}_k =
    \begin{pmatrix}
        \tilde{a}_k\\
        \tilde{a}_{-k}^\dagger
    \end{pmatrix}
\end{align}
and the $2 \times 2$ matrix $\tilde{H}_k$ is given by
\begin{align}
    \tilde{H}_k
     &=
    \begin{pmatrix}
        w_k   &r_k\\
        r_k^* &-w_k
    \end{pmatrix}\nonumber\\
     &\equiv
    \begin{pmatrix}
        \sin\theta + \cos\theta \cos(\frac{2\pi k}{N})
         &
        \cos\theta \sin(\frac{2\pi k}{N})
        \\
        \cos\theta \sin(\frac{2\pi k}{N})
         &
        -\left[ \sin\theta + \cos\theta \cos(\frac{2\pi k}{N})\right]
    \end{pmatrix}.
    \label{eq:Hk_2x2_matrix}
\end{align}
Moreover, since terms such as $\tilde{a}_0^\dagger \tilde{a}_{-0}^\dagger$ vanish due to the fermionic anticommutation relation, we obtain only diagonal terms for both $H_{k=0,N/2}$. In particular, we have
\begin{align}
    H_{k=0}
     &=
    \frac{1}{2} \sin\theta
    \Bigl(\tilde{a}_0^\dagger \tilde{a}_0
    -
    \tilde{a}_0 \tilde{a}_0^\dagger
    \Bigr) +
    \frac{1}{2} \cos\theta
    \Bigl[
        \tilde{a}_0^\dagger \tilde{a}_0
        +
        \tilde{a}_0 \tilde{a}_0^\dagger
        \Bigr]
\end{align}
and
\begin{align}
    H_{k=N/2}
     &=
    \frac{1}{2} \sin\theta
    \Bigl(\tilde{a}_{N/2}^\dagger \tilde{a}_{N/2}
    -
    \tilde{a}_{N/2} \tilde{a}_{N/2}^\dagger
    \Bigr)\nonumber\\
     &\quad
    - \frac{1}{2} \cos\theta
    \Bigl(\tilde{a}_{N/2}^\dagger \tilde{a}_{N/2} +
    \tilde{a}_{N/2} \tilde{a}_{N/2}^\dagger
    \Bigr),
\end{align}
which is diagonal in the mode $\tilde{a}_{N/2}$. Using this way of grouping the terms in the Hamiltonian, we see that, apart from the cases $k=0,N/2$, we only need to sum over the positive values $k=1,2,\ldots,N/2-1$, as the negative $-k$ are automatically included.

% ------------------------------------------------------------
\subsection{Bogoliubov transformation and diagonalization}

We now diagonalize each block Hamiltonian via a Bogoliubov transformation. We focus on the generic modes with $1 \leq k \leq N/2-1$, which appear in $2\times 2$ block form. The special cases at $k=0$ and $k=N/2$ are already diagonal as shown above.

\subsubsection{Diagonalizing the \texorpdfstring{$2\times 2$}{2 by 2} block for generic \texorpdfstring{$k$}{k}}

Because each $2\times 2$ matrix $\tilde{H}_k$ (\cref{eq:Hk_2x2_matrix}) is real and symmetric, it is diagonalizable through a real orthogonal transformation. The eigenvalues are $\pm \epsilon_k$ with

\begin{equation}
    \epsilon_k = \sqrt{w_k^2 + r_k^2}=\sqrt{1 + \sin2\theta \cos\frac{2\pi k}{N}},
    \label{eq:app:epsilonk}
\end{equation}

To determine the eigenvector corresponding to $+\epsilon_k$, we parameterize the real, normalized eigenvector as
\begin{align}
    \begin{pmatrix}
        x\\
        y
    \end{pmatrix} = \begin{pmatrix}
                        \cos(\varphi_k)\\
                        \sin(\varphi_k)
                    \end{pmatrix}.
    \label{eq:bog_positive_eigenvector_ansatz}
\end{align}
Substituting \cref{eq:bog_positive_eigenvector_ansatz} in the eigenvalue equation and solving for the ratio of components, we get
\begin{align}
    \frac{\sin(\varphi_k)}{\cos(\varphi_k)} = \tan(\varphi_k) = \frac{\epsilon_k - w_k}{r_k}.
    \label{eq:bog_ratio_sin_cos}
\end{align}
As the eigenvector to eigenvalue $-\epsilon_k$ is necessarily the real vector orthogonal to the one given in \cref{eq:bog_positive_eigenvector_ansatz}, we have that the real orthogonal matrix $U_k$ that diagonalizes $\tilde{H}_k$ is
\begin{align}
    U_k &=
    \begin{pmatrix}
        \cos(\varphi_k) &- \sin(\varphi_k)\\
        \sin(\varphi_k) &\quad\cos(\varphi_k)
    \end{pmatrix},
    \label{eq:bog_Uk_matrix}
\end{align}
Explicitly, we have $U_k^\mathsf{T} \tilde{H}_k U_k= \mbox{diag}(\epsilon_k, -\epsilon_k)$.
Moreover, we can obtain a more explicit final result for $\tan(2\varphi_k)$ by applying trigonometric identities and substituting the expressions for $\epsilon_k$, $w_k$, and $r_k$ into \cref{eq:bog_ratio_sin_cos}:
\begin{align}
    \tan2\varphi_k
     &=
    \frac{2 \tan(\varphi_k)}{1 - \tan^2(\varphi_k)}\nonumber\\
     &=
    \frac{\sin(\frac{2\pi k}{N})}{\tan\theta +\cos(\frac{2\pi k}{N})} = \frac{r_k}{w_k}.
    \label{eq:bog_tan_phi_k_final}
\end{align}


\subsubsection{Mapping to Bogoliubov quasiparticles}

This diagonalization at the matrix level defines a canonical transformation on the fermionic operators. Recall that
\begin{align}
    \tilde{\alpha}_k = \begin{pmatrix}
                           \tilde{a}_k\\
                           \tilde{a}_{-k}^\dagger
                       \end{pmatrix}.
\end{align}
The Bogoliubov transformation defined by
\begin{align}
    \hat{\alpha}_k = U_k^\mathsf{T} \tilde{\alpha}_k =
    \begin{pmatrix}
        \cos(\varphi_k) \tilde{a}_k
        +
        \sin(\varphi_k) \tilde{a}_{-k}^\dagger
        \\
        -\sin(\varphi_k) \tilde{a}_k
        +
        \cos(\varphi_k) \tilde{a}_{-k}^\dagger
    \end{pmatrix},
\end{align}
diagonalizes the Hamiltonian block $\tilde{H}_k$, i.e.,
\begin{align}
    \hat{\alpha}_k^\dagger
    \begin{pmatrix}
        + \epsilon_k &0\\
        0            &- \epsilon_k
    \end{pmatrix}
    \hat{\alpha}_k
    = + \epsilon_k \hat{a}_k^\dagger \hat{a}_k
    -
    \epsilon_k \hat{a}_{-k} \hat{a}_{-k}^\dagger,
\end{align}
for each $k\neq 0,N/2$.


\subsubsection{Diagonalized system Hamiltonian and ground-state energy}

Putting together all modes, including the special cases at $k=0$ and $k=N/2$, the Hamiltonian becomes
\begin{align}
    H_S
     &= \sum_{k=0}^{N/2} \epsilon_k h_k,
    \label{eq:bogoliubov_HS_diag}
\end{align}
where $\epsilon_k=\epsilon_{-k}$ and for the special cases $k=0$ or $k=N/2$ (those modes appear purely diagonally) we have $\hat{a}_k=\hat{a}_{-k}^\dagger$. The operators $h_k$ are given by  $h_k=\hat{a}^\dagger_k \hat{a}_k-\hat{a}_{-k}\hat{a}_{-k}^\dagger$ for $k=1,\ldots,N/2-1$ and $h_k=\hat{a}_k^\dagger \hat{a}_k-\hat{a}_k \hat{a}_k^\dagger$ for $k=0,N/2$.

Consequently, the ground state of $H_S$ is the vacuum state annihilated by all $\hat{a}_k$, i.e.,
\begin{align}
    \hat{a}_k\ket{\Psi_{GS}}=0
    \quad
    \text{for all }
    k,
\end{align}
and the ground-state energy is
\begin{align}
    E_{GS} = - \frac{1}{2}
    \sum_{k=-N/2+1}^{N/2}
    \epsilon_k,
\end{align}
with $\epsilon_k$ given in \cref{eq:app:epsilonk}.

% ------------------------------------------------------------
\subsection{Bath Hamiltonian}

The system is coupled to a bath consisting of $N$ independent fermionic sites with Hamiltonian:
\begin{equation}
    H_B = \frac{\Delta}{2}\sum_{n=1}^N \left(b_n^\dagger b_n - b_n b_n^\dagger\right),
    \label{eq:bath-hamiltonian}
\end{equation}
where $b_n$ ($b_n^\dagger$) denotes the bath fermionic annihilation (creation) operator at site $n$, and $\Delta$ is the bath energy splitting. The bath is initialized in its ground state $\rho_B = \ket{\Omega}\bra{\Omega}$ at the beginning of each cooling cycle, and this ground state is annihilated by each $b_n$, i.e., $b_n\ket{\Omega}=0$.

We now transform \cref{eq:bath-hamiltonian} to momentum space, following the same steps as in the system Hamiltonian derivation. We use the same (inverse) Fourier transformation as before and obtain
\begin{align}
    H_B = \frac{\Delta}{2}
    \sum_{k=-N/2+1}^{N/2}
    (\tilde{b}_k^\dagger \tilde{b}_k -\tilde{b}_k \tilde{b}_k^\dagger).
    \label{eq:bath-hamiltonian-momentum-derived}
\end{align}
We now organize the sum in \cref{eq:bath-hamiltonian-momentum-derived} to pair positive and negative modes, yielding $2\times 2$ blocks for generic $k$ and diagonal terms for $k=0, N/2$:
\begin{align}
    H_B
     &=
    \sum_{k=1}^{N/2-1}
    \tilde{\beta}_k^\dagger \hat{H}_k \tilde{\beta}_k+
    \frac{\Delta}{2}
    (\tilde{b}_0^\dagger \tilde{b}_0 - \tilde{b}_0 \tilde{b}_0^\dagger)\nonumber\\
     &\quad  +
    \frac{\Delta}{2}
    (\tilde{b}_{N/2}^\dagger \tilde{b}_{N/2} - \tilde{b}_{N/2} \tilde{b}_{N/2}^\dagger),
\end{align}
where
\begin{align}
    \tilde{\beta}_k = \begin{pmatrix}
                          \tilde{b}_k\\
                          \tilde{b}_{-k}^\dagger
                      \end{pmatrix}, \quad
    \hat{H}_k = \begin{pmatrix}
                    \Delta &0\\
                    0      &-\Delta
                \end{pmatrix}.
\end{align}


% ------------------------------------------------------------
\subsection{Coupling to the bath}

The system-bath coupling is assumed to be translation-invariant and extends up to a range of $nn$ nearest neighbors. It is given by
\begin{equation}
    {V}_{SB} = g \sum_{n=1}^N \sum_{j=-nn}^{nn} \left[\left(\lambda_j a_n^\dag {b}_{n+j} + i \mu_j a_n {b}_{n+j}\right) + \text{h.c.}\right],
    \label{eq:system-bath-coupling}
\end{equation}
where $g$ is the coupling strength, and $\lambda_j,\mu_j\le 1$ are dimensionless coupling constants to modes for different neighbor distances $j$.

To analyze this coupling in momentum space, we substitute the Fourier transforms of the system and bath operators (\cref{eq:fourier_def_ann}) into \cref{eq:system-bath-coupling}. After simplifying, this yields:
\begin{align}
    V_{SB} &= g \sum_{k=-N/2+1}^{N/2} \bigg[\left(\sum_{j=-nn}^{nn} \lambda_j e^{-i \frac{2\pi kj}{N}}\right) \tilde{a}_k^\dagger \tilde{b}_k\\
           &\quad + i\left(\sum_{j=-nn}^{nn} \mu_j e^{-i \frac{2\pi kj}{N}}\right) \tilde{a}_{-k} \tilde{b}_k + \text{h.c.}\bigg]
\end{align}
Organizing $V_{SB}$ into blocks pairing $k$ with $-k$ modes, we can write:
\begin{equation}
    V_{SB} = \sum_{k=0}^{N/2} \tilde{\alpha}_k^\dagger v_{SB,k} \tilde{\alpha}_k,
    \label{eq:app:HSBMomentum}
\end{equation}
where for each positive $k$ (except $k=0,N/2$), we define the four-component vector:
\begin{equation}
    \tilde{\alpha}_k = \begin{pmatrix}
        \tilde{a}_k\\
        \tilde{a}_{-k}^\dagger\\
        \tilde{b}_k\\
        \tilde{b}_{-k}^\dagger
    \end{pmatrix}.
\end{equation}



In \cref{sec:multifreq_longtime} of the main text, we consider only local couplings ($nn=0$) with $\lambda_0=\mu_0=1$, for which we have
\begin{equation}
    \label{eq:local_coupling_nn0}
    V_{SB} = g\sum_{k=-N/2+1}^{N/2} [\tilde{a}_k^\dagger \tilde{b}_k + i\tilde{a}_k \tilde{b}_{-k} + \tilde{b}_k^\dagger \tilde{a}_k - i\tilde{b}_{-k}^\dagger \tilde{a}_k^\dagger].
\end{equation}
That is, in this case we have for $1 \leq k \leq N/2-1$ the matrices $v_{SB,k}$ are given by
\begin{equation}
    v_{SB,k} = g\begin{pmatrix}
        0  &0  &1 &i\\
        0  &0  &i &-1\\
        1  &-i &0 &0\\
        -i &-1 &0 &0
    \end{pmatrix}.\label{eq:vSB_k}
\end{equation}
and for $k=0$ and $k=N/2$ we have
\begin{equation}
    v_{SB,0} = v_{SB,N/2} = v_{SB,k}/2
    \label{eq:vSB_0}
\end{equation}
with the corresponding vectors
\begin{equation}
    \tilde{\alpha}_0 = \begin{pmatrix}
        \tilde{a}_0\\
        \tilde{a}_0^\dagger\\
        \tilde{b}_0\\
        \tilde{b}_0^\dagger
    \end{pmatrix},\quad \tilde{\alpha}_{N/2} = \begin{pmatrix}
        \tilde{a}_{N/2}\\
        \tilde{a}_{N/2}^\dagger\\
        \tilde{b}_{N/2}\\
        \tilde{b}_{N/2}^\dagger
    \end{pmatrix}.
\end{equation}


\subsection{The total Hamiltonian}

The total Hamiltonian can now be written as the following sum over Hamiltonians of pairs of modes, $(k,-k)$:
\begin{equation}
    H_{SB} = H_S + H_B + V_{SB} = \sum_{k=0}^{N/2} \hat{\alpha}_k^\dagger h_{SB,k} \hat{\alpha}_k.\\
    \label{eq:app:HSB}
\end{equation}
for both local and non-local coupling. Let us first consider the case of local coupling ($nn=0$), as discussed in \cref{sec:multifreq_longtime}, where for generic $k$ ($1 \leq k \leq N/2-1$) we have
\begin{align}
    h_{SB,k} &=
    \begin{pmatrix}
        w_k &r_k  &g      &gi\\
        r_k &-w_k &gi     &-g\\
        g   &-gi  &\Delta &0\\
        -gi &-g   &0      &-\Delta
    \end{pmatrix},
\end{align}
with
\begin{align}
    w_k &= \sin\theta + \cos\theta\cos(2\pi k/N),\\
    r_k &= \cos\theta\sin(2\pi k/N).
\end{align}
For the special cases $k=0$ and $k=N/2$, we multiply the matrices $h_{S,k}$, $h_{B,k}$, and $v_{SB,k}$ by $1/2$ as shown in \cref{eq:vSB_0}, and the entries $w_k$ and $r_k$ are evaluated at the corresponding values of $k=0$ and $k=N/2$.
For the case where coupling is not local (i.e., $nn>0$), the derivation is similar. However, the entries of the matrices depend on the values of various coupling constants $\lambda_j$ and $\mu_j$. The final result for this case is presented below. % neighbor distances.

\subsection{Block diagonalization of the total Hamiltonian}


We apply the Bogoliubov transformation derived earlier for the system modes to the full Hamiltonian. The transformation matrix $U_k$ for the system part is extended to act on the full four-component space:
\begin{equation}
    \mathcal{U}_k =
    \begin{pmatrix}
        U_k &0\\
        0   &I_2
    \end{pmatrix}
\end{equation}
where $I_2$ is the $2\times 2$ identity matrix and $U_k$ is given in \cref{eq:bog_Uk_matrix}.
The transformed matrices $\hat{h}_{SB,k} = \mathcal{U}_k^\mathsf{T} h_{SB,k} \mathcal{U}_k$ for generic $k$ are given by
\begin{align}
    \hat{h}_{SB,k} &=
    \begin{pmatrix}
        \epsilon_k          &0                   &g e^{i\varphi_k}   &ig e^{i\varphi_k}\\
        0                   &-\epsilon_k         &ig e^{-i\varphi_k} &-g e^{i\varphi_k}\\
        g e^{-i\varphi_k}   &-ig e^{-i\varphi_k} &\Delta             &0\\
        -ig e^{-i\varphi_k} &-g e^{-i\varphi_k}  &0                  &-\Delta
    \end{pmatrix}.
\end{align}
For the special cases $k=0$ and $k=N/2$, we follow the same procedure but note the extra factor of 1/2. The final transformed Hamiltonian takes the block-diagonal form:
\begin{equation}
    H_{SB} = \sum_{k=0}^{N/2} \hat{\alpha}_k^\dagger \hat{h}_{SB,k} \hat{\alpha}_k,
\end{equation}
where $\hat{\alpha}_k = \mathcal{U}_k^\mathsf{T} \tilde{\alpha}_k$ are the transformed operators, and $\hat{h}_{SB,k}$ is the block Hamiltonian derived in \cref{subsec:total_hamiltonian} of the main text.

If the nearest neighbor distance extends beyond local couplings ($nn>0$), the procedure is the same and the Hamiltonian per each block $(k,-k)$ is given by
\begin{align}
    \hat{h}_{SB,k} &=
    \begin{pmatrix}
        \epsilon_k &0           &gA_k   &gB_k\\
        0          &-\epsilon_k &gB_k   &-g A_k\\
        g A_k^*    &g B_k^*     &\Delta &0\\
        gB_k^*     &-g A_k^*    &0      &-\Delta
    \end{pmatrix},\label{eq:hsb_momentum_space_nn>0}
\end{align}
where the coupling coefficients are:
\begin{align}
    A_k &=\sum_{j=-nn}^{nn}\left(\cos(\varphi_k)\lambda_j+i\sin(\varphi_k)\mu_j\right)e^{-i\frac{2\pi jk}{N}}
    \label{eq:Ak in hsb_k}\\
    B_k &=\sum_{j=-nn}^{nn}\left(-\sin(\varphi_k)\lambda_j+i\cos(\varphi_k)\mu_j\right)e^{-i\frac{2\pi jk}{N}}.
    \label{eq:Bk in hsb_k}
\end{align}

For the case $nn=0$, $\lambda_0=\mu_0=1$, we have $A_k = e^{i\varphi_k}$ and $B_k = ie^{-i\varphi_k}$.


==> newCoolingAppB.tex <==
\section{Symmetries in case the coupling is non-local, i.e.~\texorpdfstring{$nn>0$}{nn>0}}
\label{app:theta_mapping}

As explained in \cref{subsec:sys_model} of the main text, in case of local coupling ($nn=0$) and $\lambda_0=\mu_0=1$, we can restrict $\theta$ to the region $[0,\pi/2]$. Here, we show that this also holds for the general case of non-local couplings. To this end, we show that systems with $\theta$ outside this region can be mapped to equivalent systems within the region by appropriate transformations of the coupling parameters.

Let us first analyze the mapping $\theta \rightarrow -\theta$. Under this transformation, the system Hamiltonian $H_S$ [\cref{eq:system_hamiltonian_realspace}] undergoes sign changes in its terms. This transformation can be implemented through a mapping of fermionic operators where mode $k$ is mapped to $k\pm N/2 \mod N$. Specifically, $k=0$ is mapped to $k'=N/2$, mode $k=1$ to $k'=-N/2+1$, and vice versa, mode $k=-N/2+1$ to $k'=1$, etc.
For the system-bath coupling [\cref{eq:system-bath-coupling_realspace}], this transformation requires the coupling constants to transform as:
\begin{align}
    \lambda_j' &= \lambda_j(-1)^j,\\
    \mu_j'     &= \mu_j(-1)^j.
\end{align}

In the special case where $nn=0$, this mapping reduces to the symmetry explained in \cref{subsec:sys_model} of the main text since the only relevant coupling constants are $\lambda_0$ and $\mu_0$, which remain unchanged.

The other symmetry appears when considering the transformation $\theta'=\pi+\theta$. In this case, the two modes being mapped to one another are the same, $k'=k$, since this change in $\theta$ keeps the energy of each mode invariant. Specifically, we have:
\begin{align}
    \epsilon_k(\theta+\pi) &= \epsilon_k(\theta),\\
    \varphi_k(\theta+\pi)  &= \varphi_k(\theta),
\end{align}
where the second equation follows from $\tan(\theta+\pi)=\tan(\theta)$.
Since these quantities remain invariant, there is no need to modify the coupling constants $\lambda_j$ and $\mu_j$ under this transformation.

By combining these two symmetries, we can map any value of $\theta$ from the region $[-\pi/2,3\pi/2]$ to a value within the range $[0,\pi/2]$, with appropriate adjustments to the coupling constants. This extends the result mentioned in \cref{subsec:sys_model} of the main text to the general case of non-local coupling ($nn > 0$).

==> newCoolingAppC.tex <==
\section{Noise}
\label{app:secIV_noise}

In this appendix, we present the details about the cooling map in the presence of depolarizing noise as described in \cref{sec:adding_decoherence}. We start by showing that the cooling and noise Lindbladians commute and then derive the cooling map and the modified states on which the map acts.

\subsection{Proof that \texorpdfstring{$\mathcal{L}_C$}{LC} commutes with \texorpdfstring{$\mathcal{L}_E$}{LE}}
\label{app:LcCommuteLe}


The total evolution during a cooling cycle is governed by the master equation:
\begin{equation}
    \dot \rho_{SB} = \mathcal{L}_C(\rho_{SB}) + \mathcal{L}_E(\rho_{SB}),
\end{equation}
where $\mathcal{L}_C(\rho) = -i [H_{SB},\rho]$ generates the unitary evolution under the system-bath Hamiltonian $H_{SB}$, and $\mathcal{L}_E$ represents the environmental noise:
\begin{equation}
    \mathcal{L}_E = \kappa\sum_{n=1}^N \left[\mathcal{L}_{a_n} + \mathcal{L}_{a_n^\dagger} + \mathcal{L}_{b_n} + \mathcal{L}_{b_n^\dagger}\right].
    \label{eq:app:LE_def}
\end{equation}
Here, $\mathcal{L}_O(\rho) = O\rho O^\dagger - \frac{1}{2}\{O^\dagger O,\rho\}$.
Using the fermionic anticommutation relations, we can simplify the noise Lindbladian to:
\begin{equation}
    \mathcal{L}_E(\rho) = \kappa\sum_{n=1}^N \left[ (a_n\rho a_n^\dagger + a_n^\dagger\rho a_n - \rho) + (b_n\rho b_n^\dagger + b_n^\dagger\rho b_n - \rho) \right].
    \label{eq:LE_explicit_app}
\end{equation}


We will prove that $[\mathcal{L}_C, \mathcal{L}_E] = 0$.
The commutation relation is equivalent to showing that $\mathcal{L}_E$ is invariant under the unitary evolution generated by $H_{SB}$, i.e., that the following equality holds for $U(t) = e^{-i H_{SB} t}$:
\begin{equation}
    \mathcal{L}_E^I(\rho) \equiv U(t)^\dagger \mathcal{L}_E(U(t) \rho U(t)^\dagger) U(t) = \mathcal{L}_E(\rho),\label{eq:LE_invariance_condition}
\end{equation}
where $\mathcal{L}_E^I$ denotes the noise Lindbladian in the interaction picture with respect to $H_{SB}$. This can be easily seen as follows. Let us denote by $R=(a_1,\ldots, a_n, b_1,\ldots, b_n, a_1^\dagger,\ldots, a_n^\dagger, b_1^\dagger,\ldots, b_n^\dagger)$. Then, the fermionic anticommutation relations read $\{R_i,R_j^\dagger\}=\delta_{i,j}$. As the Hamiltonian $H_{SB}$ is quadratic in the fermionic operators, its action transforms $R$ into a vector $S=A R$, for some $4n\times 4n$ dimensional matrix $A$. Furthermore, $S$ has to obey the fermionic anticommutation relations, i.e., $\{S_i,S_j^\dagger\}=\delta_{i,j}$, which is fulfilled iff $A$ is unitary. Using this, it is straightforward to see that
\begin{equation}
    \mathcal{L}_E(\rho) =\sum_{i=1}^{4n}\left[ (R_n\rho R_n^\dagger  - 2 \rho) \right]=\sum_{i=1}^{4n}\left[ (S_n\rho S_n^\dagger  - 2 \rho) \right]= \mathcal{L}_E^I(\rho), \label{eq:LE_invariance_proof}
\end{equation}
which proves the statement. This commutation relation allows us to factorize the time evolution as follows
\begin{align}
    e^{(\mathcal{L}_C + \mathcal{L}_E)t} &= e^{\mathcal{L}_C t} e^{\mathcal{L}_E t} = e^{\mathcal{L}_E t} e^{\mathcal{L}_C t}.
\end{align}
Therefore, the noisy cooling map $\mathcal{N}$ for one cycle can be expressed as applying the noise evolution $e^{\mathcal{L}_E t}$ first, followed by the noiseless cooling map $\mathcal{E}$ (which corresponds to $e^{\mathcal{L}_C t}$ and tracing over the bath):
\begin{align}
    \mathcal{N}(\rho_S)
     &= \tr_B\left[e^{(\mathcal{L}_C + \mathcal{L}_E)t}(\rho_S \otimes \rho_B)\right] \nonumber\\
     &= \tr_B\left[e^{-iH_{SB}t} (\tilde{\rho}_S \otimes \tilde{\rho}_B) e^{i H_{SB}t}\right],
\end{align}
where $\tilde{\rho}_S = e^{\mathcal{L}_E t}(\rho_S)$ is the system density matrix evolved under noise, and $\tilde{\rho}_B = e^{\mathcal{L}_E t}(\rho_B)$ is the evolved bath state.


In order to determine $\tilde{\rho}_B$ we first note that the initial state of the bath is its ground state, i.e., $\rho_B = \ket{\Omega}\bra{\Omega} = \bigotimes_{n=1}^N \ket{0_n}\bra{0_n}$. Note further that $\mathcal{L}_E$ acts independently on each site $n$. Hence, we can determine $\tilde{\rho}_B = e^{\mathcal{L}_E t}(\rho_B)$ by focusing on bath modes individually.
We consider a single bath mode $b_n$ and solve the master equation $\dot{\rho}_{B,n} = \kappa (\mathcal{L}_{b_n} + \mathcal{L}_{b_n^\dagger}) \rho_{B,n}$ for the density matrix $\rho_{B,n}$ of site $n$, with initial condition $\rho_{B,n}(0) = \ket{0_n}\bra{0_n}$. Let $\rho_{B,n} = \begin{pmatrix} \rho_{00} & \rho_{01} \\ \rho_{10} & \rho_{11} \end{pmatrix}$. The equations for the matrix elements are:
\begin{equation}
    \dot{\rho}_{00} = \kappa (\rho_{11} - \rho_{00})
    = \kappa (1 - 2\rho_{00})
\end{equation}
which has the solution (recall that $\rho_{00}(0) = 1$),
\begin{align}
    \rho_{00}(t) = 1-\rho_{11}(t) = \frac{1+e^{-2\kappa t}}{2}.
\end{align}


Similarly, it is straightforward to see that the coherence terms $\rho_{01}$ and $\rho_{10}$ decay exponentially under $\mathcal{L}_E$. This can be easily seen by solving their respective ODEs, leading to
\begin{equation}
    \rho_{01}(t)=\rho_{01}(0)e^{-\kappa t}.
\end{equation}
with $\rho_{01}(0)=0$.
Thus, the bath state after the noise evolution for time $t$ is
\begin{align}
    \tilde{\rho}_B &= e^{\mathcal{L}_E t}(\ket{\Omega}\bra{\Omega})\nonumber\\
                   &= \bigotimes_{n=1}^N \left( \frac{1+e^{-2\kappa t}}{2}\ket{\Omega}\bra{\Omega}+\frac{1-e^{-2\kappa t}}{2}\ket{1}\bra{1} \right).
\end{align}
This mixed state is then used as the initial state of the bath for the cooling cycle.

Since the form of the noise is the same and independent for both the system and the bath, the time evolution equation for $\rho_S$ under noise alone is the same as that of the bath:
\begin{align}
    \frac{d\tilde{\rho}_S}{dt} &= \mathcal{L}_E(\tilde{\rho}_S) = \kappa\sum_{n=1}^N \left[\mathcal{L}_{a_n}(\tilde{\rho}_S) + \mathcal{L}_{a_n^\dagger}(\tilde{\rho}_S)\right].
\end{align}
The solution to this equation gives us $\tilde{\rho}_S = e^{\mathcal{L}_E t}(\rho_S(0))$ at time $t$, which is then used as the initial state for the cooling process in the numerical simulations reported in \cref{sec:multifreq_longtime,sec:nn_cooling} of the main text.

Contrary to the bath, we cannot separate the different $n$ modes and calculate the effect of the noise on each of them independently, so one would need to switch to momentum space and act on the 4 by 4 matrices for each $k,-k$ block of $\rho_S$. Additionally, we should take into account that the initial state of the system is different for every cycle. However, as will be shown in \cref{app:Single_freq steady state}, approximations can be made to simplify the noisy map $\mathcal{N}(\rho)$ so this calculation is not needed.


\subsection{Noisy map in momentum space}

For numerical simulations, it is convenient to express the master equation derived above in momentum space. The noise Lindbladian in momentum space is obtained by transforming the real-space Lindbladian $\mathcal{L}_E = \kappa\sum_{n=1}^N \left[\mathcal{L}_{a_n} + \mathcal{L}_{a_n^\dagger} + \mathcal{L}_{b_n} + \mathcal{L}_{b_n^\dagger}\right]$ using the Fourier transform. Since the Fourier transform is a unitary transformation (a specific canonical transformation), and $\mathcal{L}_E$ is invariant under canonical transformations as shown in \cref{app:LcCommuteLe}, the form remains the same but with momentum operators:
\begin{align}
    \mathcal{L}_E = \kappa\sum_{k=-N/2+1}^{N/2} \left[\mathcal{L}_{\tilde{a}_k} + \mathcal{L}_{\tilde{a}_k^\dagger} + \mathcal{L}_{\tilde{b}_k} + \mathcal{L}_{\tilde{b}_k^\dagger}\right].
\end{align}
Due to the translational invariance of both the system Hamiltonian and the noise, the density matrix in momentum space decomposes into a tensor product over momentum modes $(k,-k)$: $\tilde{\rho}_S = \bigotimes_{k=0}^{N/2} \tilde{\rho}_S^{(k)}$ and $\tilde{\rho}_B = \bigotimes_{k=0}^{N/2} \tilde{\rho}_B^{(k)}$.

Due to the block-diagonal structure of both $H_{SB}$ and $\mathcal{L}_E$ in momentum space, the noisy cooling map in momentum space can therefore be written as:
\begin{align}
    \mathcal{N}(\rho_S)         &= \bigotimes_{k=0}^{N/2} \mathcal{N}_k(\rho_S^{(k)}) \mbox{ with }\\
    \mathcal{N}_k(\rho_S^{(k)}) &= \tr_{B_k}\left[e^{-ih_{SB,k}t}(\tilde{\rho}_S^{(k)} \otimes \tilde{\rho}_B^{(k)})e^{i h_{SB,k}t}\right],
\end{align}
where $h_{SB,k}$ is the block Hamiltonian for momentum mode $k$ derived in \cref{subsec:total_hamiltonian} of the main text (and \cref{app:Hk_derivation}), and for each momentum mode pair $k$, the bath state evolves to:
\begin{align}
    \tilde{\rho}_B^{(k)} = &\left(\frac{1+e^{-2\kappa t}}{2}\ket{\Omega}\bra{\Omega}+\frac{1-e^{-2\kappa t}}{2}\ket{1}\bra{1} \right)^{\otimes 2}.
\end{align}
This formulation allows for efficient numerical implementation of the noisy cooling process, where each momentum block can be treated independently, as used in the simulations presented in \cref{sec:multifreq_longtime,sec:nn_cooling}.

==> newCoolingAppD.tex <==

\section{Derivation of convergence times}
\label{app:secIV_calculations}


In this appendix, we provide a detailed derivation of the scaling of the cooling time presented in \cref{sec:cooling_times_and_ss}.
We start out in \cref{subsec:zeroth_order_mixing_time} by showing how the distance between the state obtained after applying $n$ times a general completely positive map~(CPM), ${\cal E}$, to some input state and the unique stationary state of the CPM converges with $n$. In \cref{subsec:global_convergence} we then use the fact that the stationary state of our cooling map factorizes in momentum space to derive a bound on the cooling rate. In \cref{subsec:energy_convergence}, we determine the number of cycles required to achieve an energy density which is close to that of the stationary state.


\subsection{Mixing time and convergence to stationary state for generic CPM}
\label{subsec:zeroth_order_mixing_time}

In order to determine how fast the system converges to the stationary state, we use the relation between the transfer matrix and the CPM. Given a linear map, $T$, with $T(\cdot)=\sum_j L_j \cdot R_j$, the transfer matrix is defined as $\hat{T}=\sum_j L_j \otimes R_j^T$. The relation between the transfer matrix, $\hat{T}$, and the Choi-state, $E$ is $\hat{T}=d E^T$, where $E^T$ is defined via $\langle m,n|E^T | k,l\rangle=\langle m,k|E|n,l\rangle$, i.e., $\hat{T}=d E^{T_B} \text{SWAP}$, where $T_B$ denotes the partial transpose with respect to system $B$ and SWAP is defined via $\text{SWAP} |k,l\rangle=|l,k\rangle$ and $d$ denotes the dimension. It is straightforward to see that the concatenation of maps, $T_1 \circ T_2$ corresponds to the transfer matrix $\hat{T}_1 \cdot \hat{T}_2$. Note that in general $\hat{T}$ will not be Hermitian. Using the Jordan decomposition of $\hat{T}$, one can determine the action of $T^n$. Let us consider the dense set of non-defective matrices, which will be the generic case~\footnote{For non-diagonalizable (defective) matrices, the Jordan decomposition still allows us to analyze the convergence.}. For those we have that the algebraic multiplicity of each eigenvalue coincides with its geometric multiplicity.
They can be written as $\hat{T}=\sum_k \lambda_k |R_k\rangle \langle L_k|$, where $\langle L_k|R_l\rangle =\delta_{k,l}$, i.e., with biorthogonal right and left eigenvectors of $\hat{T}$. From this decomposition we have $\hat{T}^n = \sum_k \lambda_k^n |R_k\rangle \langle L_k|$. The corresponding map can be written as: $\mathcal{E}(\rho) = \sum_{m} \lambda_m \tilde{\mathcal{E}}_m(\rho)$, where $\tilde{\mathcal{E}}_m$ corresponds to the transfer matrix $ |R_m\rangle \langle L_m|$.


Therefore, we have
\begin{align}
    \mathcal{E}^n(\rho) = \sum_{m} \lambda_m^n \tilde{\mathcal{E}}_m(\rho).
    \label{eq:spectral_decomposition_map_n}
\end{align}
For a cooling process to be effective and for it to converge to a unique steady state, all eigenvalues other than $\lambda_1 = 1$ must satisfy $|\lambda_m| < 1$ for $m > 1$~\footnote{Recall that we consider here the case where we have a unique stationary state.} As the number of iterations $n$ increases, the terms $\lambda_m^n$ with $|\lambda_m| < 1$ will approach zero.

We can separate the term corresponding to $\lambda_1 = 1$ from the sum in \cref{eq:spectral_decomposition_map_n} to obtain
\begin{align}
    \mathcal{E}^n(\rho) &= \tilde{\mathcal{E}}_1(\rho) + \sum_{m=2} \lambda_m^n \tilde{\mathcal{E}}_m(\rho)\nonumber\\
                        &= \rho_\text{ss} + \sum_{m=2} \lambda_m^n \tilde{\mathcal{E}}_m(\rho).
\end{align}

To analyze the convergence to the steady state, we consider the difference between the evolved state $\mathcal{E}^n(\rho)$ and the steady state $\rho_\text{ss}$:
\begin{align}
    \mathcal{E}^n(\rho) - \rho_\text{ss} = \sum_{m=2} \lambda_m^n \tilde{\mathcal{E}}_m(\rho).
    \label{eq:difference_evolved_steadystate}
\end{align}
The rate of convergence is determined by how quickly this difference goes to zero as $n \to \infty$, which is governed by the eigenvalue $\lambda_2$, with second largest eigenvalue absolute value. Let us assume that there are more eigenvalues, $\lambda_2, \lambda_2', \lambda_2'', \ldots$ with the same magnitude $|\lambda_2|$. We denote the corresponding maps by $\tilde{\mathcal{E}}_2'$, etc. Then, for large $n$, we can approximate the difference as:
\begin{align}
    \mathcal{E}^n(\rho) - \rho_\text{ss} &\approx \lambda_2^n \tilde{\mathcal{E}}_2(\rho) + (\lambda_2')^n \tilde{\mathcal{E}}_2'(\rho) + (\lambda_2'')^n \tilde{\mathcal{E}}_2''(\rho) + \cdots \nonumber\\
                                         &= \lambda_2^n \left[ \tilde{\mathcal{E}}_2(\rho) + \tilde{\mathcal{E}}_2'(\rho) + \tilde{\mathcal{E}}_2''(\rho) + \cdots \right],
    \label{eq:difference_evolved_steadystate_approx}
\end{align}
where we have factored out $\lambda_2^n$ and redefined $\tilde{\mathcal{E}}_2'$, etc.~with a possible phase.
To quantify the convergence, we take the one-norm of the difference:
\begin{align}
    \|\mathcal{E}^n(\rho) - \rho_\text{ss}\|_1 &\approx \left\| \lambda_2^n \left[ \tilde{\mathcal{E}}_2(\rho) + \tilde{\mathcal{E}}_2'(\rho) + \tilde{\mathcal{E}}_2''(\rho) + \mathcal{O}\left(\frac{\lambda_3^n}{\lambda_2^n}\right)\right] \right\|_1 \nonumber\\
                                               &= |\lambda_2|^n \left\| \tilde{\mathcal{E}}_2(\rho) + \tilde{\mathcal{E}}_2'(\rho) + \tilde{\mathcal{E}}_2''(\rho) + \cdots \right\|_1\nonumber\\
                                               &= C |\lambda_2|^n = C e^{-n\alpha},
    \label{eq:norm_difference_evolved_steadystate}
\end{align}
with a constant $C$ and the cooling rate $\alpha$ as:
\begin{align}
    C      &= \left\| \tilde{\mathcal{E}}_2(\rho) + \tilde{\mathcal{E}}_2'(\rho) + \tilde{\mathcal{E}}_2''(\rho) + \cdots \right\|_1,\\
    \alpha &= -\log |\lambda_2| > 0.
    \label{eq:constant_C_definition}
\end{align}

Let us apply these bounds now to the map $\mathcal{E}_k$. More specifically, we consider a mode pair $(k,-k)$ and define a mode-specific cooling rate $\alpha_k = -\log |\lambda_k|$, where $\lambda_k$ is the second-largest eigenvalue of the map $\mathcal{E}_k$ in absolute value. This gives us the convergence:
\begin{equation}
    \|\mathcal{E}_k^n(\rho_k) - \sigma_k\|_1 \leq e^{-\alpha_k n},
    \label{eq:mode_convergence_rate}
\end{equation}
where $\sigma_k$ is the (unique) steady state of the map $\mathcal{E}_k$.
The number of cycles required to reach the steady state for mode $k$ is then:
\begin{equation}
    n^c_k = \alpha_k^{-1}.
    \label{eq:n0k_app}
\end{equation}

\subsection{Convergence of cooling map}
\label{subsec:global_convergence}

We now analyze the convergence of the global state $\mathcal{E}^n(\rho)$ to the global steady state $\rho_{S}^\text{ss} = \bigotimes_{k=0}^{N/2} \sigma_k$. Due to translational invariance, the cooling map $\mathcal{E}$ and its steady state can be decomposed into a tensor product of maps $\mathcal{E}_k$ and their corresponding steady states $\sigma_k$ for each momentum mode pair $k$. That is,
\begin{align}
    \mathcal{E}=\bigotimes_{k=0}^{N/2} \mathcal{E}_k, \quad \rho_{S}^\text{ss} = \bigotimes_{k=0}^{N/2} \sigma_k.
\end{align}
We assume the initial state is also a product state over the modes, $\rho_S = \bigotimes_{k=0}^{N/2} \rho_k$.

Our goal is to determine the global cooling time, i.e., how many cycles are needed for the global state $\mathcal{E}^n(\rho)$ to approach the global steady state $\rho_{S}^\text{ss} = \bigotimes_k \sigma_k$. We quantify this convergence using the one-norm distance
\begin{align}
    \|\mathcal{E}^n(\rho)-\bigotimes_k \sigma_k\|_1 = \|\bigotimes_{k=0}^{N/2}\mathcal{E}_k^n(\rho_k)-\bigotimes_{k=0}^{N/2}\sigma_k\|_1.
\end{align}
To bound this global distance, we will use the Kaleidoscope inequality. Let us denote by $\chi_i$ the tensor product state where the first $i$ modes are evolved and the remaining modes are in their steady state. That is,
\begin{equation}
    \chi_i = \left( \bigotimes_{j=0}^{i-1}\mathcal{E}_j^n(\rho_j) \right) \otimes \left( \bigotimes_{l=i}^{N/2} \sigma_l \right).
\end{equation}
We define $\chi_0 = \bigotimes_{k=0}^{N/2}\sigma_k$ and $\chi_{N/2+1} = \bigotimes_{k=0}^{N/2}\mathcal{E}_k^n(\rho_k)$. Then we can write the global distance as a telescoping sum:
\begin{align}
    \|\bigotimes_{k=0}^{N/2}\mathcal{E}_k^n(\rho_k)-\bigotimes_{k=0}^{N/2}\sigma_k\|_1
     &= \|\chi_{N/2+1} - \chi_0\|_1 \nonumber\\
     &= \left\| \sum_{i=1}^{N/2+1} (\chi_i - \chi_{i-1}) \right\|_1 \nonumber\\
     &\le \sum_{i=1}^{N/2+1} \|\chi_i - \chi_{i-1}\|_1,
\end{align}
where the inequality follows from the triangle inequality for the one-norm. Using that $\|\tau \otimes \rho - \tau \otimes \sigma\|_1 = \|\rho - \sigma\|_1$, we obtain
\begin{equation}
    \|\chi_i - \chi_{i-1}\|_1 = \|\mathcal{E}_{i-1}^n(\rho_{i-1}) - \sigma_{i-1}\|_1.
\end{equation}

Therefore, the global distance is bounded by the sum of the distances for each mode (also called the Kaleidoscope inequality):
\begin{align}
    \|\mathcal{E}^n(\rho)-\bigotimes_{k=0}^{N/2}\sigma_k\|_1 &\leq \sum_{k=0}^{N/2} \|\mathcal{E}_k^n(\rho_k)-\sigma_k\|_1.
\end{align}
Using \cref{eq:mode_convergence_rate}, we have:
\begin{align}
    \|\mathcal{E}^n(\rho) - \bigotimes_{k=0}^{N/2}\sigma_k\|_1 &\leq \sum_{k=0}^{N/2} e^{-\alpha_k n}.
\end{align}
To find a system-size independent cooling rate, we define the global cooling rate $ \alpha = \inf_N \min_k \alpha_k$. Assuming $\alpha > 0$, we can bound the sum by taking the minimum rate $\alpha$:
\begin{align}
    \sum_{k=0}^{N/2} e^{-\alpha_k n} \le \sum_{k=0}^{N/2} e^{-\alpha n} = (N/2 + 1) e^{-\alpha n} < N e^{-\alpha n},
\end{align}
where we have neglected $\mathcal{O}(1)$ factors for simplicity, focusing on the scaling with $N$. Thus, we obtain the global convergence rate:
\begin{equation}
    \|\mathcal{E}^n(\rho)-\bigotimes_{k=0}^{N/2}\sigma_k\|_1 \leq N e^{-\alpha n}.
\end{equation}
This shows that to reach a state that is $\epsilon$-close (in one-norm distance) to the steady state, i.e., $\|\mathcal{E}^n(\rho)-\rho_{S}^\text{ss}\|_1 \le \epsilon$, we need a number of cycles $n^c$ such that $N e^{-\alpha n^c} \approx \epsilon$, or equivalently,
\begin{equation}
    n^c \approx \frac{1}{\alpha} \log\left(\frac{N}{\epsilon}\right).
\end{equation}
Therefore, if $\alpha > 0$ (which is generally the case away from the phase transition at $\theta = \pi/4$), the number of cycles required to reach the steady state grows logarithmically with the system size $N$.

\subsection{Convergence of energy density}
\label{subsec:energy_convergence}

Next, we analyze the convergence of the relative energy by examining the convergence of the energy density. The error in the energy density after $n$ cycles can be bounded by
\begin{align}
    \left|\frac{1}{N}\sum_{k=0}^{N/2} \tr\left(\epsilon_k h_k \left[\mathcal{E}_k^n(\rho_k)- \sigma_k\right]\right)\right|\nonumber\\
    \le \frac{1}{N}\sum_{k=0}^{N/2} \left|\tr\left(\epsilon_k h_k \left[\mathcal{E}_k^n(\rho_k)- \sigma_k\right]\right)\right|,
\end{align}
by using the triangle inequality $|\tr(A+B)| \le |\tr(A)| + |\tr(B)|$.
Then, we use the inequality $|\tr(XY)| \le \|X\| \|Y\|_1$, where $\|X\|$ is the operator norm of $X$. We choose $X = \epsilon_k h_k$ and $Y = \mathcal{E}_k^n(\rho_k)- \sigma_k$ and will use the convergence of the state differences in the 1-norm as established in \cref{eq:mode_convergence_rate}.


The matrix $h_k = \hat{a}^\dagger_k \hat{a}_k-\hat{a}_{-k}\hat{a}_{-k}^\dagger$ has eigenvalues $\pm 1$ and thus operator norm $\|h_k\| = 1$.
Then, we have $\|\epsilon_k h_k\| = \epsilon_k$. Therefore, we bound:
\begin{align}
    \left|\tr\left(\epsilon_k h_k \left[\mathcal{E}_k^n(\rho_k)- \sigma_k\right]\right)\right|
     &\le \|\epsilon_k h_k\| \|\mathcal{E}_k^n(\rho_k)- \sigma_k\|_1 \nonumber\\
     &= \epsilon_k \|\mathcal{E}_k^n(\rho_k)- \sigma_k\|_1 \nonumber\\
     &\le \epsilon_k e^{-\alpha_k n},
\end{align}
by using the bound on mode convergence $\|\mathcal{E}_k^n(\rho_k)-\sigma_k\|_1 \le e^{-\alpha_k n}$ from \cref{eq:mode_convergence_rate}.

Substituting this back into the sum for the energy density error, we get the following bound
\begin{align}
    \frac{1}{N}\sum_{k=0}^{N/2} \left|\tr\left(\epsilon_k h_k \left[\mathcal{E}_k^n(\rho_k)- \sigma_k\right]\right)\right|
     &\le \frac{1}{N}\sum_{k=0}^{N/2} \epsilon_k e^{-\alpha_k n} \nonumber\\
     &\le \frac{1}{N}(\max_k \epsilon_k) \sum_{k=0}^{N/2} e^{-\alpha_k n} \nonumber\\
     &\le (\max_k \epsilon_k) e^{-\alpha n} \frac{N/2 + 1}{N} \nonumber\\
     &\le C e^{-\alpha n},
\end{align}
where in the last three steps we have taken the maximum value of $\epsilon_k$, used the minimum cooling rate $\alpha$, and $C = \max_k \epsilon_k$ is a constant of order $\mathcal{O}(1)$ since $\epsilon_k$ are mode energies and are bounded.
To achieve an energy density error of $\epsilon$, we need $C e^{-\alpha n^c} \approx \epsilon$, which gives
\begin{align}
    n^c &\approx \frac{1}{\alpha} \log\left(\frac{C}{\epsilon}\right)\nonumber\\
        &\approx \frac{1}{\alpha} \log\left(\frac{1}{\epsilon}\right),
\end{align}
neglecting the constant term $\frac{\log C}{\alpha}$. This shows that if $\alpha > 0$, the number of cycles required to reach a certain energy density error $\epsilon$ is independent of the system size $N$, scaling only logarithmically with the desired precision $\epsilon$.

If $\alpha = 0$, which can happen at a phase transition (e.g., at $\theta = \pi/4$ in our model), the cooling time scaling will depend on how the minimum cooling rate $\alpha_k$ approaches zero as the system size $N$ increases. If $\alpha$ decreases polynomially with $N$, the cooling time will scale polynomially with $N$.
